P-score: A Publication-based Metric for Academic Productivity

In this work we propose a metric to assess academic productivity based on publication outputs. We are interested in knowing how well a research group in an area of knowledge is doing relatively to a pre-selected set of reference groups, where each group is composed by academics or researchers. To assess academic productivity we propose a new metric, which we call P-score. Our metric P-score assigns weights to venues using only the publication patterns of selected reference groups. This implies that P-score does not depend on citation data and thus, that it is simpler to compute particularly in contexts in which citation data is not easily available. Also, preliminary experiments suggest that P-score preserves strong correlation with citation-based metrics.

==> ack.tex <==
\section*{Acknowledgments}

%\vspace{0.4cm}

%This work was partially sponsored the Brazilian National Institute of Science and Technology for the Web (grant MCT/ CNPq 573871/2008-6), and by the authors' individual grants and scholarships from CNPq, FAPEMIG and FAPERJ. We thank Leonardo Santos Resende for his contributions to this project.


==> basic-considerations.tex <==
%\subsection{Basic Considerations}

{\color{Gray}

An important assumption of our proposal is that we can reasonably identify a set
of the most prestigious programs (that we refer to as the {\em top reference set}) 
in a given area and that we have access to the venues where the faculty members
of these programs publish.
Notice that distinct top reference sets might be considered, which will lead to distinct 
R-Score results. The important points to emphasize here are: (a) R-Score provides a comparison 
of publication output in view of a pre-selected set of top reference programs and 
(b) selecting a dozen or so top reference programs in a given area can be done much more 
objectively and with much smaller effort than weighting hundreds of publication venues in 
that area, or computing citation counts for papers in those venues. 

Regarding R-Score computation, it 
is important to emphasize that there is no need to access the contents of the
papers published by the faculty members of these programs and the citations to
their work.  
Also, there is no need to rank the programs in the {\em top reference set}.
What is required is simply to count the number of publications
by the faculty members of programs 
in the chosen {\em top reference set} at different venues.

Two issues that immediately arise is how to choose the programs in the {\em top reference set}
and how many programs we need to include in this set.
We argue that it is not difficult to identify a few dozens programs that would be
reasonable candidates to the {\em top reference set}. 
If we ask a set of senior professors in a given area of knowledge to name, for instance,
the top $10$ programs 
in the world in their area, we expect that a large fraction of all selected programs 
will be included in a large fraction of each of the professor's list.
For instance, if the area chosen is Computer Science, graduate programs run by 
departments at the Massachusetts Institute of Technology, Univerity of California at Berkeley, 
Carnegie Mellon University, and Stanford University will most likely be included 
in any {\em top reference set} list. 
In fact, a brief search in world wide academic rankings would support such claim.
We postpone the choice of the cardinality of the {\em top reference set} 
for future sections where we also study the sensitivity of the results we report
to the size of the {\em top reference set}.

In what follows, we describe the methodology we propose.
It is based on a {\em role model} concept, in which one should take as model
the most reputable individuals in our society.
We start by stating our main assumptions.

\begin{asp}
\label{asp:dep-fac}
The reputation of a graduate program is strongly influenced by the reputation of its faculty, 
which is largely dependent on their publication track records. 
\end{asp}
As a consequence of this assumption, the graduate programs in the {\em top reference set} employ the most prestigious faculty.
The more prestigious is a program the better chances it has to attract the most prominent Ph.D. graduates and
senior renowned scientists. 

%The venues where the faculty in the departments in the {\em top reference set} are
%the most prestigious.
\begin{asp}
\label{asp:fac-ven}
A researcher, or member of a graduate program, conveys reputation to a venue proportionally to its own reputation.
\end{asp}
This assumption is a consequence of what we call the role-model effect.
Reputable scientists usually choose prestigious venues to publish at and, as
such, the reputation of a venue is positively correlated with the reputation of the individuals that publish in
that venue.
As more prestigious researchers of an area choose a venue to publish their work, the venue becomes increasingly 
known by peer researchers and, as a consequence, attracts even more distinguished researchers and
young scientists, building up its reputation.   

\begin{asp}
\label{asp:ven-fac}
The reputation of a faculty member is positively correlated with the reputation of the venues in which he/she
publishes.
\end{asp}
One of the most used metrics to promote a faculty member in any reputable department or graduate program 
is the number of papers in prestigious venues where the faculty under consideration publishes. 
Clearly, if a given scientist has a reasonable number of papers in the most prestigious venues
then it is reasonable to assume he/she is a prestigious scientist.

The three assumptions above form the cornerstone of our reputation-based ranking model.
Our model is inspired by the {\em eigenvalue centrality} metrics for complex networks
\cite{Newman-book}, which operate quite similarly to Page Rank \cite{Meyer-pagerank06}.
This metric is obtained by assuming
that the relative importance (or reputation)
of a node in a network is proportional to the importance of the nodes that point to it.
In addition, a given node distributes its importance uniformly among the nodes it points to.
We map these ideas to obtain a ranking model for a set of venues.

}



==> chart.tex <==

%\usepackage{pgfplots}
%\pgfplotsset{compat=1.8}

%\begin{figure}\centering
\begin{tikzpicture}
\begin{axis}
[ ybar,
  xlabel={Top-$n$, Economics},
  ylabel={Fraction of Top-$n$ in both rankings},
  xtick=data,
  xticklabels from table={chart.dat}{XLabel},
  bar width=16pt,
  width=0.5*\textwidth,
  x tick label style={font=\small,align=right,rotate=0},
  y tick label style={font=\small,align=right,rotate=0},
  enlarge x limits=0.2,
  y domain=0:1,
  ymin=0,ymax=1,
]
\addplot table
[ x=XPos,
  y=YPos,
] 
{chart.dat};
\end{axis}
\end{tikzpicture}
%\end{figure}


